DeepFacePencil: Creating Face Images from Freehand Sketches

In this paper, we explore the task of generating photo-realistic face images from hand-drawn sketches. Existing image-to-image translation methods require a large-scale dataset of paired sketches and images for supervision. They typically utilize synthesized edge maps of face images as training data. However, these synthesized edge maps strictly align with the edges of the corresponding face images, which limit their generalization ability to real hand-drawn sketches with vast stroke diversity. To address this problem, we propose DeepFacePencil, an effective tool that is able to generate photo-realistic face images from hand-drawn sketches, based on a novel dual generator image translation network during training. A novel spatial attention pooling (SAP) is designed to adaptively handle stroke distortions which are spatially varying to support various stroke styles and different levels of details. We conduct extensive experiments and the results demonstrate the superiority of our model over existing methods on both image quality and model generalization to hand-drawn sketches.

==> algorithm_train.tex <==
% !TeX root = SketchFace.tex

In order to train our model more stably, we introduce a multi-stage training schedule. At the first stage, we use edge-aligned sketches and real images to train $G_a$ and $D$ without loss function related to $G_m$. At the second stage, we train SAP and the encoder of $G_m$ and $D$ from scratch while fixing weights of other parts. Note that the residual blocks and the decoder of $G_m$ that share weights with those of $G_a$ keep unchanged in this stage. At the last stage, we finetune the whole model with the overall objective in Eq.~\ref{eqn:new_minmax_game}. 
